ColdGuess: A General and Effective Relational Graph Convolutional Network to Tackle Cold Start Cases

Low-quality listings and bad actor behavior in online retail websites threatens e-commerce business as these result in sub-optimal buying experience and erode customer trust. When a new listing is created, how to tell it has good-quality? Is the method effective, fast, and scalable? Previous approaches often have three limitations/challenges: (1) unable to handle cold start problems where new sellers/listings lack sufficient selling histories. (2) inability of scoring hundreds of millions of listings at scale, or compromise performance for scalability. (3) has space challenges from large-scale graph with giant e-commerce business size. To overcome these limitations/challenges, we proposed ColdGuess, an inductive graph-based risk predictor built upon a heterogeneous seller product graph, which effectively identifies risky seller/product/listings at scale. ColdGuess tackles the large-scale graph by consolidated nodes, and addresses the cold start problems using homogeneous influence1. The evaluation on real data demonstrates that ColdGuess has stable performance as the number of unknown features increases. It outperforms the lightgbm2 by up to 34 pcp ROC-AUC in a cold start case when a new seller sells a new product . The resulting system, ColdGuess, is effective, adaptable to changing risky seller behavior, and is already in production

==> Tables/intro.tex <==
% added line by christos, for write-access test

\section{Introduction}
% Each year Amazon receives hundreds of millions of product related complaints globally. These degrade the customer shopping experience and erode customer trust.
% This also has a big negative impact on the Amazon brand.
% These complaints are categorized into eight types, such as Expired, Used Sold as New, Defective, Damaged, Wrong Item Sent, Version Mismatch and Other Negative Product Experience. 

Low-quality listings and bad seller behaviors in e-commerce website often lead to product complaints and erode customer trust. This causes a big negative impact on e-commerce website brand. Companies like Amazon, eBay and Alibaba, have spent lots of effort to combat low-quality \ASIN listings~\cite{chen2015big, hui2016reputation}. 
%
However, it is still challenging to detect a low quality \ASIN listing among millions of normal listings. It is even more challenging when there is little historical information associated with a listing, i.e., the cold start problem.

%To mitigate these limitations and provide a perfect user experience, we developed \method, a graph neural network based complaint detector which predicts the likelihood of an offer listing\footnote{we use offer, listings, and offer listings interchangeably in the paper.} to have customer complaints in the future. The prediction results can be used to prevent low-quality listings from surfacing to customers.

% Traditional machine learning methods (e.g. logistic regression, support vector
% machines~\cite{tong2001support}, boosting tree~\cite{ke2017lgbm}, etc.) learn models to capture signals~\cite{phua2010comprehensive}. However, these methods face two limitations: (1) inability to leverage seller-seller and seller-\ASIN\footnote{Product is a generic term. A \ASIN could be sold by multiple sellers. A seller and \ASIN pair determines an offer listing.} linkage information (e.g., sellers are associated if they share the same information or similar characteristics.), which is valuable as risky sellers and offers are often found clustered;%\footnote{For example, majority of sellers who share the same information with a risky seller are also found risky.};
% and (2) unable to model new sellers/offers, namely, the cold start problem, where listings from new sellers contribute to about a quarter of complaints. There lacks sufficient history for traditional models to identify a risk. 

% In order to leverage linkage information, \method constructs a seller-\ASIN graph by connecting sellers who possess associated information or characteristics or listing same \ASINs and uses relational graph convolutional network (RGCN)~\cite{schlichtkrull2018modeling} to encode neighborhood information of sellers and \ASINs. This allows risk propagation from existing sellers to new sellers through neural message passing~\cite{gilmer2017neural}. To address the cold start problem, \method combines neural message passing with feature propagation. Specifically, \method uses RGCN model to implicitly propagate existing seller features to new sellers and uses edge feature propagation to explicitly propagate offer listing history information to new listings.

Heuristic or rule-based detection methods heavily depend on historical information and human effort, which are not flexible enough to follow the fast moving e-commerce society. 
%
Traditional machine learning methods (e.g. logistic regression, boosting tree~\cite{ke2017lgbm}, etc.) face two limitations: (1) inability to leverage seller-seller and seller-\ASIN\footnote{Product is a generic term. A \ASIN could be sold by multiple sellers. A seller and \ASIN pair determines an offer listing.} linkage information (e.g., sellers are associated if they share the same information or similar characteristics.) and (2) unable to model new sellers/offers (the cold start problem) - listings from new sellers contribute to about a quarter of complaints. However, they lack sufficient history for traditional models to identify as risky. Linkage information has proven to be valuable as risky sellers and offers are often found clustered\footnote{For example, majority of sellers who share the same information with a risky seller are also found risky.}. As Amazon continuously expands to new countries, the cold start problem becomes more common and critical.

To overcome these limitations, we propose \method, a graph neural network based complaint detector which predicts the likelihood of an offer listing\footnote{we use offer, listings, and offer listings interchangeably in the paper.} to have customer complaints in the future. %The prediction results can be used to prevent low-quality listings from surfacing to customers.


\method leverages the node connectivity information embedded in a seller-\ASINg graph~\footnote{Within a Seller-\ASINg graph, sellers are connected if they possess associated information or characteristics. Sellers and ~\ASINs are connected if there exists an associated listing.} through neural message passing~\cite{gilmer2017neural}, which allows risk propagation from existing sellers to new sellers. 
By using relational graph convolutional network (RGCN)~\cite{schlichtkrull2018modeling}, \method establishes informative graph embeddings for sellers and ~\ASINs, which are used by the complaint detector.
It utilizes the heterogeneity of the seller-\ASINg graph to improve the model expressiveness.
\method leverages the edge connectivity information through edge feature propagation, which allows risk propagation from existing offer listings to new offer listings.

%This approach leverages the connectivity information embedded in the graph, which allows risk propagation from existing sellers to new sellers through neural message passing~\cite{gilmer2017neural} and thus addresses the cold start problem. Additionally, the graph neural network layers~\cite{schlichtkrull2018modeling, kipf2016semi} establish informative graph embeddings for seller and product, which can be utilized by downstream predictive systems (e.g., anomaly detection, risky seller cluster detection, etc.).


%Additionally, the graph neural network layers~\cite{schlichtkrull2018modeling, kipf2016semi} establish informative graph embeddings for seller and \ASIN, which can be utilized by downstream predictive systems (e.g., anomaly detection, risky seller cluster detection, etc.). 

% By leveraging graph convolutional network~\cite{kipf2016semi,schlichtkrull2018modeling} which captures local graph structure and feature information through neural message passing~\cite{gilmer2017neural}, \method can easily leverage the linkage information as well as the feature information from the neighbors of a new seller or \ASIN to solve the cold start problem. The risk signals will be propagated to new sellers through message passing. Additionally, \method enriches an offer's edge feature by concatenating its feature with a summary of its neighbors' edge features. Additionally, the network layers establish feature embeddings for sellers and ASINs which can be utilized by downstream predictive systems (e.g., anomaly detection, risky seller cluster detection, etc.). 

We evaluated \method on a full spectrum of sample data and three simulated cold start scenarios (i.e. new offers, new sellers, and new sellers who sell new \ASIN). We compared its performance with lgbm, an algorithm often excel in classification problems, as well as with Graph+lgbm, a sequential model which first fills missing values using one-hop propagation and then feeds the output to lgbm. We found \method outperforms both lgbm and graph+lgbm in all cold start cases. Its predominance over lgbm and graph+lgbm increases with the increasing number of missing features. As shown in Figure~\ref{fig:intro}, \method outperforms both lgbm and graph+lgbm by up to 34\% absolute AUC in the extreme cold start scenario when a new seller sells a new \ASIN. %It has 20\% to 10 times relative improvement in average precision \footnote{measured by PC AUC} across different complaint types. 

\begin{figure}[t]
\centering
  \includegraphics[width=0.8\linewidth]{Figures/2020-11_seller_asin.png}
  \label{fig:sub1}
\caption{\method vs. benchmark models evaluated on new sellers who sell new \ASIN case using data as of 2020/11}
\label{fig:intro}
\end{figure}

The main contributions and advantages of \method are:

% \begin{enumerate}
%     \item Previous GNN models in CTPS mainly focused on homogeneous graphs/features, and are sub-optimal in the heterogeneous setting. We proposed PC-Detector framework allows risk propagation across heterogeneous graph in a highly multi-relational data set. 
%     \item In the state-of-art RGCN, missing values on edge features cannot be inferred from their neighbors since aggregation and updates only happen on node features. To deal with the missing values on edge features, We augmented an offers' edge features by concatenating it with its neighbors' edge features. An edge's neighbor edge is defined as edges connected to that offer's head and tail nodes. 
%     \item We found RGCN has superb performance and outperforms LGBM in cold start cases, though it cannot beat LGBM when evaluated on overall data. 
% \end{enumerate}
\begin{itemize}
\item \textbf{Holistic:} The inductive \method framework can handle (a) \textit{Dynamic heterogeneous graphs built on highly relational data} with millions of nodes, tens of millions of edges, and massive node and edge features.
%both node and edge features on the graph. 
%Previous GNN models in production was either transductive or mainly focused on homogeneous graphs without features, and are sub-optimal in the heterogenous setting. \method framework works for heterogeneous graph constructed from a highly multi-relational data set and allows node feature propagation over different node types and edge types. %Note from xiangsx: This statement is not valid, thus I comment it out. 
% \item \textit{Cold start problem}. \method achieves stable performance with increasing number of missing features on new offer/seller/ASIN scenarios. It outperforms LGBM by up to \textbf{30\%} in an extreme cold start case where a seller sells a new ASIN.
(b) \textit{Missing values on edge feature} In the state-of-art RGCN, missing values on edge features cannot be inferred from their neighbors since aggregation and updates only happen on the nodes. To deal with that, we augmented an offers’ edge features by concatenating it and its neighbors'.
% by concatenating an edge feature and a summary of its neighbors' edge features.

\item \textbf{Effective}, especially for \textit{Cold Start Problem}: \method achieves stable performance with increasing number of missing features in new offer/seller/\ASIN scenarios. It outperforms lgbm by up to \textit{35.9\%} absolute AUC in the extreme cold start case where a new seller sells a new \ASIN. 
%improves its performance from basic RGCN setting by concatenating edge feature with its neighbor's edge features. In the state-of-art RGCN, missing values on edge features cannot be inferred from their neighbors since aggregation and updates only happen on node features. To deal with the missing values on edge features, we augmented an offers' edge features by concatenating it with its neighbors' edge features. An edge's neighbor edge is defined as edges connected to that offer's head and tail nodes.
%\item \textbf{Effective:} \method has superb performance and outperforms lgbm in cold start cases. 
\item \textbf{Fast:} 
\method can scale to a business size graph with tens of millions of edges. It takes only 2 minutes to make 1MM+ predictions. The training on a graph with 1.5MM+ offer listings takes an hour on a single GPU, and 20 minutes when distributed computing on a 4-GPU p3.8xlarge EC2 with 244G memory.  
\end{itemize}

\newcommand{\myrotate}[1]{\rotatebox{80}{#1}}
\begin{table}[t]
  \centering
  \caption{\method matches all specs, while competitors miss one or more of the features.}
  \begin{tabular}{l|cccc||c}
  \diagbox{Property}{Method}
    &\myrotate{lgbm}&\myrotate{graph+lgbm}&\myrotate{SIGN}
    &\myrotate{RGCN}&\myrotate{\method}\\
    %   Method & lgbm & graph+lgbm & SIGN & RGCN & \method \\    
      \hline
      node connectivity   &  & $\surd$ & $\surd$ & $\surd$ & $\surd$\\

      heterogeneous info. &  &         &         & $\surd$ & $\surd$ \\
      edge connectivity   &  &         &         &         & $\surd$ \\
      
  \end{tabular}
  \label{tab:ds}
\end{table}

% 

